Uniform Non-Deterministic Semantics for Ciuciura's $mbC^n$-Hierarchy

We introduce a uniform non-deterministic semantics for the hierarchy of paraconsistent systems mbC^n introduced by Ciuciura. The proposed construction generalizes Omori's three-valued semantics for mbC^1 to all systems of the hierarchy. We prove soundness and completeness of the semantics with respect to the corresponding axiomatizations and show that the consequence relations of the systems mbC^n cannot be characterized by finite deterministic matrices.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{A. Indrzejczak, T. Jarmu\.zek, M. Klonowski, \& M. Zawidzki (Eds.):\\ Twelfth International Conference on\\ Non-Classical Logics. Theory and Applications (NCL'26)\\
EPTCS 455, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.455.1}{10.4204/EPTCS.455.1}}
\pdfoutput=1

